$\textit{Dial BeInfo for Faithfulness}$: Improving Factuality of Information-Seeking Dialogue via Behavioural Fine-Tuning

Factuality is a crucial requirement in information seeking dialogue: the system should respond to the user's queries so that the responses are meaningful and aligned with the knowledge provided to the system. However, most modern large language models suffer from hallucinations, that is, they generate responses not supported by or contradicting the knowledge source. To mitigate the issue and increase faithfulness of information-seeking dialogue systems, we introduce BeInfo, a simple yet effective method that applies behavioural tuning to aid information-seeking dialogue. Relying on three standard datasets, we show that models tuned with BeInfo} become considerably more faithful to the knowledge source both for datasets and domains seen during BeInfo-tuning, as well as on unseen domains, when applied in a zero-shot manner. In addition, we show that the models with 3B parameters (e.g., Flan-T5) tuned with BeInfo demonstrate strong performance on data from real `production' conversations and outperform GPT4 when tuned on a limited amount of such realistic in-domain dialogues.

==> 111_randoms.tex <==
\iffalse
\begin{table}[!h]
\def\arraystretch{0.95}
\centering
\resizebox{0.9\linewidth}{!}{%
\begin{tabular}{l cccc}
\hline
\textbf{Model}                  & BLEU  & ROUGE & BERTS-F1 & $\mathcal{K}$-BERTS-F1 \\ \hline
Best T5-based baseline & 10.9  & 35.8  & -        & -          \\
Flan-T5-base tuned     & 14.97 & 38.80 & 69.64    & 78.46      \\
Flan-T5-base tuned+EWR & 14.9  & -     & 70.1     & 81.7       \\ \midrule 
Flan-T5-base raw       & 2.48  & 12.85 & 42.36    & 48.95      \\
Flan-T5-base+approach  & 12.52 & 36.35 & 67.67    & 69.04      \\
Flan-T5-large raw      & 3.35  & 15.44 & 48.80    & 51.23      \\
Flan-T5-large+approach & 13.66 & 37.85 & 72.04    & 70.95      \\
Flan-T5-xl raw         & 4.46  & 17.3  & 53.99    & 54.91      \\
Flan-T5-xl+approach    & 15.78 & 38.69 & 75.19    & 75.19      \\ \hline
\end{tabular}
}
\caption{results for improvement}
\label{tab: results improvement}
\end{table}


\paragraph{\approach~ for Task-Specific Tuning.}

\begin{table}[!h]
\def\arraystretch{0.95}
\centering
\resizebox{0.9\linewidth}{!}{%
\begin{tabular}{lrrrrr}
\hline
Model                  & \multicolumn{1}{c}{BLEU} & \multicolumn{1}{c}{ROUGE} & \multicolumn{1}{c}{BERTS-F1} & \multicolumn{1}{c}{K-BERTS-F1} & \multicolumn{1}{l}{K-Precision} \\ \hline
\multicolumn{6}{l}{FaithDial}                                                                                                                                                   \\
Flan-T5+EWR            & 14.9                     & \multicolumn{1}{l}{-}     & 70.1                         & 81.7                           & \multicolumn{1}{l}{-}           \\
Flan-T5 raw tuned      & 14.97                    & 38.798                    & 69.64                        & 78.46                          & 66.79                           \\
Flan-T5 approach tuned & 14.98                    & 38.434                    & 69.69                        & 78.49                          & 66.32                           \\
\multicolumn{6}{l}{TopiOCQA}                                                                                                                                                    \\
Flan-T5 raw tuned      & 36.24                    & 68.64                     & 80.94                        & 73.38                          & 83.63                           \\
Flan-T5 approach tuned & 38.75                    & 69.57                     & 81.4                         & 72.24                          & 83.64                           \\ \hline
\end{tabular}
}
\caption{results for further tuning on seen datasets}
\label{tab: results finetuning}
\end{table}



-- main results

-- "out-of-domain" results

-- tuning on smaller dataset

-- different instruction-tuned model
\fi
